A Unified Survey on Anomaly, Novelty, Open-Set, and Out-of-Distribution Detection: Solutions and Future Challenges

Machine learning models often encounter samples that are diverged from the training distribution. Failure to recognize an out-of-distribution (OOD) sample, and consequently assign that sample to an in-class label significantly compromises the reliability of a model. The problem has gained significant attention due to its importance for safety deploying models in open-world settings. Detecting OOD samples is challenging due to the intractability of modeling all possible unknown distributions. To date, several research domains tackle the problem of detecting unfamiliar samples, including anomaly detection, novelty detection, one-class learning, open set recognition, and out-of-distribution detection. Despite having similar and shared concepts, out-of-distribution, open-set, and anomaly detection have been investigated independently. Accordingly, these research avenues have not cross-pollinated, creating research barriers. While some surveys intend to provide an overview of these approaches, they seem to only focus on a specific domain without examining the relationship between different domains. This survey aims to provide a cross-domain and comprehensive review of numerous eminent works in respective areas while identifying their commonalities. Researchers can benefit from the overview of research advances in different fields and develop future methodology synergistically. Furthermore, to the best of our knowledge, while there are surveys in anomaly detection or one-class learning, there is no comprehensive or up-to-date survey on out-of-distribution detection, which our survey covers extensively. Finally, having a unified cross-domain perspective, we discuss and shed light on future lines of research, intending to bring these fields closer together.

==> Figures/C2AE.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=\linewidth]{Pictures/C2AE.pdf}
    \caption{The overall network of C2AE. As it can be seen, an AE is trained in such a way that minimizes the reconstruction error of match samples while maximizing the reconstruction error of none-match ones. At the inference time, the reconstruction error of input is computed conditioned on different match vectors, and the decision of rejection is made based on their minimum value. Also, the rejection threshold is computed based on EVT.}
    \label{fig:C2AE}
\end{figure}

==> Figures/MOOD.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=120mm]{Pictures/MOOD.pdf}
    \caption{The overall architecture of MOOD. As the figure shows, some OOD samples can be detected by applying simple low-level computations, as opposed to some others that need more complex modelings. Test time computations can be done dynamically and on demand, which significantly reduces computational cost. The figure is taken from \cite{lin2021mood}.}
    \label{fig:MOOD}
\end{figure}
